Image coding for machines: an end-to-end learned approach

Over recent years, deep learning-based computer vision systems have been applied to images at an ever-increasing pace, oftentimes representing the only type of consumption for those images. Given the dramatic explosion in the number of images generated per day, a question arises: how much better would an image codec targeting machine-consumption perform against state-of-the-art codecs targeting human-consumption? In this paper, we propose an image codec for machines which is neural network (NN) based and end-to-end learned. In particular, we propose a set of training strategies that address the delicate problem of balancing competing loss functions, such as computer vision task losses, image distortion losses, and rate loss. Our experimental results show that our NN-based codec outperforms the state-of-the-art Versa-tile Video Coding (VVC) standard on the object detection and instance segmentation tasks, achieving -37.87% and -32.90% of BD-rate gain, respectively, while being fast thanks to its compact size. To the best of our knowledge, this is the first end-to-end learned machine-targeted image codec.

==> chapters/entropy_model.tex <==
\chapter{Entropy model recap}
\label{ch:entropymodel}

\section{Arithmetic coding}
In arithmetic coding, a string of symbols will be encoded into one float number. The probability of the next symbol determines which sub-range of value that symbol will be encoded into.

\paragraph{Example} Given a dictionary of 4 symbols A, B, C, D with the probabilities in \autoref{tab:probdist}. The string ``ACD'' would be encoded as shown in \autoref{fig:ACD_encoding}.

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|}
        \hline
         Symbol & Probability \\
         \hline
         A & 0.6 \\
         B & 0.2 \\
         C & 0.1 \\
         D & 0.1 \\
         \hline
    \end{tabular}
    \caption{Probability distribution}
    \label{tab:probdist}
\end{table}

\begin{figure}[h]
  \begin{center}
      \includegraphics[width=0.8\textwidth]{figures/AC_example.png}
  \end{center}
  \caption{Encoding of ``ACD'' \cite{ac_wiki}}

  \label{fig:ACD_encoding}
\end{figure}

The arithmetic encoder and decoder need to look up on the \autoref{tab:probdist} to do their jobs. In case of ``Adaptive'' arithmetic coding, this table would change at every step according to the ``context''. The entropy model (or prior probability model) (\autoref{ssec:entropymodel}) tries to predict this table for the Arithmetic coder. The more accurate it is, the lower entropy it gets, which is lower-bounded by the entropy of the unknown actual distribution of the symbols.

\section{Entropy model - the hyperprior approach}
\label{ssec:entropymodel}
In this line of work, an encoder $\Wmodel{E}{\Tensor{x}}$ is used to transform the input image $\Tensor{x}$ into a latent tensor $\Tensor{y}$, which is subsequently quantized by $\Model{Q}{\cdot}$ to discrete value tensor $\Tensor{\hat{y}}$. During training, the quantization is approximated by additive uniform noise, in order to preserve the gradient flow, since this step produces gradient zero with respect to $\ModelWeights{E}$ almost everywhere. The approximated quantized latent is denoted with a tilde: $\Tensor{\Tilde{y}}$. 

Each element of the latent tensor is modeled by a Gaussian mixture model. In Balle's papers \cite{scale_hyperprior} and \cite{meanscale_hyperprior}, a hyperprior model is trained to predict the parameters of those Gaussian mixtures. These parameters are thus called ``hyperprior''. Once we have hyperprior, the distribution $p_{\iqlatent}$ (similar to \autoref{tab:probdist}) can be estimated for the latent tensor $\iqlatent$. Since the actual marginal distribution of $\iqlatent$ is unknown, the estimated bitrate $\Loss{rate}$ is given by cross-entropy of the marginal distribution $m_{\iqlatent}$ and $p_{\iqlatent}$:
\begin{equation}
    \begin{split}
        \Loss{rate}
        & = \mathbb{E}_{\Tensor{\hat{y}} \sim m_{\Tensor{\hat{y}} }} \left[-\log_{2} p_{\Tensor{\hat{y}}}(\Tensor{\hat{y}})\right] \\
        & = \mathbb{E}_{\Tensor{x} \sim p_{\Tensor{x}}}\left[-\log_{2} p_{\hat{\boldsymbol{y}}}(\Model{Q}{\Wmodel{E}{\Tensor{x}}})\right] \\
        & = -\sum_{x \in \mathcal{X}}\left(p_{\Tensor{x}}(\Tensor{\Tensor{x}})\log_{2} p_{\hat{\boldsymbol{y}}}(\Model{Q}{\Wmodel{E}{\Tensor{x}}})\right)
    \end{split}
    \label{eq:loss_rate}
\end{equation}

\begin{frame}{Questions}
    \color{red}
    Here come the first 2 questions:
    \begin{enumerate}
        % \item In our implementation, the \mintinline{Python}{ScaleHyperprior} and \mintinline{Python}{MeanScaleHyperprior} models take as input the latent tensor of the main encoder. Do we just use the hyper auto-encoder part from Balle's papers, or do we take also their ``main autoencoder'' part into these models?
        \item How do we  calculate the rate estimation, exactly? Because in the last line of \autoref{eq:loss_rate}, I see that we still need the probabilities from the unknown distribution of $\Tensor{x}$ (if everything I wrote there is correct). I would guess that we can assume our dataset is large enough and there's no duplicate image, therefore $p_{\Tensor{x}}(\Tensor{x}) = 1,~\forall \Tensor{x} \in \mathcal{X}_{dataset}$, and the last line of \autoref{eq:loss_rate} would become $-\sum_{x \in \mathcal{X}_{dataset}}\left(\log_{2} p_{\hat{\boldsymbol{y}}}(\Model{Q}{\Wmodel{E}{\Tensor{x}}})\right)$?.
    \end{enumerate}
    \label{question:first}
\end{frame}

\subsection{The ScaleHyperprior model}
Original paper:  \cite{scale_hyperprior}
\paragraph{Intuition:} the spatially neighboring elements of the latent representation $\Tensor{y}$ tend to vary together in their scales. Their analysis is shown in \autoref{fig:scale_dependencies}.
\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/scale_dependencies.png}
    \caption{[Courtesy of \cite{scale_hyperprior}] Left: an image from the Kodak dataset. Middle left: visualization of a subset of the latent
representation $\Tensor{y}$ of that image, learned by our factorized-prior model. Note that there is clearly
visible structure around edges and textured regions, indicating that a dependency structure exists
in the marginal which is not represented in the factorized prior. Middle right: standard deviations
$\Tensor{\hat{\sigma}}$ of the latents as predicted by the model augmented with a hyperprior. Right: latents $\Tensor{y}$ divided
element-wise by their standard deviation. Note how this reduces the apparent structure, indicating
that the structure is captured by the new prior.
}
    \label{fig:scale_dependencies}
\end{figure}
\paragraph{Assumptions:} 
The values for each element of the approximately quantized latent tensor $\Tensor{\Tilde{y}}$ can be modeled by a zero-mean Gaussian:
\begin{equation*}
    \Tilde{y}_i = \mathcal{N}(0, \sigma_i) * \mathcal{U}(-\frac{1}{2}, \frac{1}{2}), 
\end{equation*}
where standard deviation (``scale'') $\sigma_i$ is predicted by the hyperprior model.
Therefore the probability of $\hat{y}_i$ can be given by a closed-form formula:
\begin{equation*}
p_{\iqlatent}\left(\hat{y}_{i} \mid \hat{\sigma}_{i}\right)=p_{\tqlatent}\left(\hat{y}_{i} \mid \hat{\sigma}_{i}\right)=\left(\mathcal{N}\left(0, \hat{\sigma}_{i}\right) * \mathcal{U}\left(-\frac{1}{2}, \frac{1}{2}\right)\right)\left(\hat{y}_{i}\right)=\int_{\hat{y}_{i}-1 / 2}^{\hat{y}_{i}+1 / 2} \mathcal{N}\left(y \mid 0, \hat{\sigma}_{i}\right) \mathrm{d} y
\end{equation*}
\paragraph{The ``hyperprior model''} in general includes another auto-encoder structure stacked on top of the main auto-encoder that takes the latent $\Tensor{\hat{y}} (inference)|\Tensor{\Tilde{y}} (training)$ as input. The ``hyperprior'' tensor $\Tensor{\hat{\sigma}}|\Tensor{\Tilde{\sigma}}$ has the same dimensional as that of the quantized latent tensor $\Tensor{\hat{y}}|\Tensor{\Tilde{y}}$, meaning each element $\hat{y_i}|\Tilde{y_i}$ of $\Tensor{\hat{y}}|\Tensor{\Tilde{y}}$ will get one scale prediction $\hat{\sigma_i}|\Tilde{\sigma_i}$.  The whole pipeline is shown in \autoref{fig:hyperprior_overview}.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/hyperprior_pipeline.png}
    \caption{[Courtesy of \cite{scale_hyperprior}] Hyperprior approach overview }
    \label{fig:hyperprior_overview}
\end{figure}
\paragraph{Performance:} Better than any other preceding NN-based method, still behind BPG (HEVC based)\cite{bpg}.


\begin{frame}{Questions}
    \color{red}
    The next not-so-good question: what does $\mathcal{N}\left(0, \hat{\sigma}_{i}\right) * \mathcal{U}\left(-\frac{1}{2}, \frac{1}{2}\right)$ looks like? I could only imagine $\mathcal{N}\left(0, \hat{\sigma}_{i}\right) + \mathcal{U}\left(-\frac{1}{2}, \frac{1}{2}\right)$, and didn't find the right keyword to google this :D
\end{frame}

\subsection{The MeanScaleHyperprior model}
Original paper \cite{meanscale_hyperprior}

Extending the ``Scale hyperprior'' \cite{scale_hyperprior}, this work captures more correlations in the latent representation $\Tensor{y}$ by:
\begin{itemize}
    \item Switching from zero-mean Gaussian scale model to Gaussian mixture model. That means the hyperprior will also include the means of the Gaussians, instead of assuming them to be zero-mean. The output hyperprior tensor therefore has double the number of channels for both means and scales.
    \item Adding an autoregressive context model and another NN model to combine this information with the output of the hyper-autoencoder in order to produce the final hyperprior. The whole pipeline is shown in \autoref{fig:meanscale_overview}. 
\end{itemize}
The probability of $\iqlatent$, given the learned parameters then becomes:
\begin{equation*}
\begin{array}{c}
p_{\hat{y}}\left(\iqlatent \mid \iqhyperlatent, \boldsymbol{\theta}_{h d}, \boldsymbol{\theta}_{c m}, \boldsymbol{\theta}_{e p}\right)=\prod_{i}\left(\mathcal{N}\left(\mu_{i}, \sigma_{i}^{2}\right) * \mathcal{U}\left(-\frac{1}{2}, \frac{1}{2}\right)\right)\left(\hat{y}_{i}\right) \\
\text { with } \mu_{i}, \sigma_{i}=g_{e p}\left(\boldsymbol{\psi}, \boldsymbol{\phi}_{i} ; \boldsymbol{\theta}_{e p}\right), \boldsymbol{\psi}=g_{h}\left(\iqhyperlatent ; \boldsymbol{\theta}_{h d}\right), \text { and } \phi_{i}=g_{c m}\left(\hat{y}_{<i} ; \boldsymbol{\theta}_{c m}\right)
\end{array}
\end{equation*}
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/meanscalehyperpior_overviewpng.png}
    \caption{[Courtesy of \cite{meanscale_hyperprior}] Their combined model jointly optimizes an autoregressive component that predicts latents
from their causal context (Context Model) along with a hyperprior and the underlying autoencoder.
Real-valued latent representations are quantized (Q) to create latents ($\tqlatent$) and hyper-latents ($\iqhyperlatent$), which
are compressed into a bitstream using an arithmetic encoder (AE) and decompressed by an arithmetic
decoder (AD). The highlighted region corresponds to the components that are executed by the receiver
to recover an image from a compressed bitstream.}
    \label{fig:meanscale_overview}
\end{figure}

\paragraph{Intuitions:} Without the zero-mean assumption of the Gaussian mixture, the predicted distribution of $\iqlatent$ would require smaller scale parameters, be more accurate, thus improves the compression rate. Additionally, combining the information stream from the context model with one from the hyper-autoencoder, in the authors' words, is beneficial from two perspectives:
\begin{itemize}
    \item Context model can provide more information without giving up bitrate because it's autoregressive.
    \item The hyper-autoencoder can ``look into the future'' to provide more useful information.
\end{itemize}
The authors provided visualizations of the results. They compressed an input image with their trained models and extracted the latents for the channel with highest entropy. Their analysis is shown in \autoref{fig:meanscale_dependencies}.
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/meanscale_dependencies.png}
    \caption{[Courtesy of \cite{meanscale_hyperprior}] Each row corresponds to a different model variant and shows information for the channel with the highest entropy. The visualizations show that more powerful models reduce the prediction error, require smaller scale parameters, and remove structure from the normalized latents, which directly translates into a more accurate entropy model and thus higher compression rates. Their entropy model assumes that latents are conditionally independent given the hyperprior, which implies that the normalized latents, i.e. values with the predicted mean and scale removed, should be closer to i.i.d. Gaussian noise.}
    \label{fig:meanscale_dependencies}
\end{figure}
\paragraph{Performance:} Even better than BPG \cite{bpg}

\begin{frame}{Questions}
    \color{red}
    The last question: I didn't find any detail on the so-called ``adaptive number of quantization bits'' in the paper. I'm aware that some channels on the latent tensor might be turned off accordingly to the choice of value for $\lambda$, but how does the model quantize the latent tensor without us giving it the specific number of levels?
\end{frame}



==> chapters/related_work.tex <==
\section{Related work}
\label{sec:related_work}

In order to directly optimize for computer vision tasks, \cite{vcm_feature_based}
and \cite{adapting_JPEGXS} propose standard-compliant methods that preserve the 
standard coded bitstream format.
The authors of \cite{vcm_feature_based} reformulate the conventional 
rate-distortion optimization (RDO) in VVC by replacing pixel-based 
distortion metrics with feature-based distortion metrics, which consequently 
guides the encoder to reduce the distortion of the features in the first layers 
of the task network, thus improves the coding efficiency. 
Authors of \cite{adapting_JPEGXS} on the other hand fine-tune the weights of 
JPEG XS ``High'' profile %\cite{jpegxs}
for task performance. 
Although the above methods manage to improve the task performance, they do not 
aim to completely replace the conventional pipeline for human-oriented coding, 
instead they only add an incremental capability to the system.

The use of neural networks (NN) to aid or completely replace the traditional 
image codec has been actively studied recently.
In \cite{jointlearnedvvc}, a CNN post-processing filter is used to further 
enhance the image quality. Some other proposals seek to effectively 
model the distribution of the data that is encoded/decoded by a lossless codec. 
To this end, autoregressive models such as \cite{pixelCNN} are used 
to model the context awareness without additional bitrate consumption while 
\cite{srec} manages to hierarchically learn the distribution through downsampled 
input at multiple scales.
In \cite{meanscale_hyperprior}, the authors 
propose end-to-end pipelines for image \textit{transform coding}, %  \cite{transformcoding}
where the image's latent representation and its distribution are entropy encoded 
instead using hierarchical learned \textit{hyperprior}.
Our work can be viewed as an extension of \cite{meanscale_hyperprior}, in which 
the main targeted end-users are task neural networks, and the main coder is 
substituted by a more capable one.

Regarding the problem of multi-objective training, 
\cite{lossweighting_overview} 
discuss the importance of loss weighting and 
propose new methods for dynamic loss balancing, as opposed to fixed weighted 
losses.
These methods, though promising, do not directly offer full control over the 
priorities of the objectives, which is a desired feature in our case.
% In \cite{weightupdate_paper}, inference-time 
% fine-tuning schemes is proposed, aimed at obtaining better compression rates, 
% while \cite{jpegai_paper} extensively studies latent tensor overfitting.
% However, as these methods target human consumption, they are only useful for 
% enhancing the fidelity in pixel domain, where ground-truth at encoder-side is 
% easily available (the uncompressed image itself) and no manually-generated 
% labels are required.
In this paper we address the issue of inference-time fine-tuning for machines, 
and improve the rate-distortion performance by fine-tuning the latent 
representation with respect to a proxy objective instead.


==> chapters/training.tex <==
\section{Training}
\label{ch:training}
